TVShowGuess: Character Comprehension in Stories as Speaker Guessing

We propose a new task for assessing machines' skills of understanding fictional characters in narrative stories. The task, TVShowGuess, builds on the scripts of TV series and takes the form of guessing the anonymous main characters based on the backgrounds of the scenes and the dialogues. Our human study supports that this form of task covers comprehension of multiple types of character persona, including understanding characters' personalities, facts and memories of personal experience, which are well aligned with the psychological and literary theories about the theory of mind (ToM) of human beings on understanding fictional characters during reading. We further propose new model architectures to support the contextualized encoding of long scene texts. Experiments show that our proposed approaches significantly outperform baselines, yet still largely lag behind the (nearly perfect) human performance. Our work serves as a first step toward the goal of narrative character comprehension.

==> experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
%%%%%%%%%%%%%%%%  Evaluation  %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Evaluation Part I: QA System Ablation}
We evaluate the overall Book QA system, and the individual modules on NarrativeQA. 
% Appendix \ref{app:append_full_results} reports the full results of our extensive experiments, where we achieve the best performance across all of the metrics.

\medskip
\noindent\textbf{Implementation Details:}
For rankers, we initialize with \texttt{bert-base-uncased}.
% \footnote{https://github.com/huggingface/transformers}. 
% The distant supervision algorithm finds the best performance at $\alpha$$=$0.7, $\beta$$=$0.3 and $\sigma$$=$8 (Section~\ref{ssec:model_ranker}).
For readers, we use \texttt{bert-base-uncased}, \texttt{gpt2-medium}, \texttt{bart-large} and \texttt{T5-base}. The readers use top-3 retrieved passages as inputs, except for the FiD reader which uses top-10, making the readers have comparable time and space complexities.
% \footnote{We use top-10 so that different readers have similar time and space complexities.}
% We use two V100 GPUs. 

\begin{table}[t!]%[width=\textwidth]
    \small
    \centering
    % \setlength{\tabcolsep}{3pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1} % Default value: 1
    \begin{tabular}{lcccccc} 
        \toprule
        \multirow{2}{*}{\bf System} & \multicolumn{2}{c}{\bf FRIENDS}& \multicolumn{2}{c}{\bf TBBT}\\
         & \bf dev & \bf test & \bf dev & \bf test \\ 
        \midrule
        Random \\
        BART-LM & \\
        BERT-avg & \\
        MultiRowBERT & 72.39 & 54.55	 \\
        \quad + Multitask & 76.82 & 64.18	 \\
        \midrule
        Human$^{*}$ & 98.68 & 89.82 \\
        \bottomrule
    \end{tabular}
    \vspace*{-2mm}
    \caption{{Overall
    performance (\%) on our \datasetname task. 
    (*) Human evaluation was conducted on a subset of the dataset.}}
    % The dagger ($^\dagger$) indicates significance with p-value < 0.01.}}
    \vspace*{-3mm}
    \label{tab:reader_model_performance}
\end{table}

\subsection{Overall Performance of Book QA}
We first show the positions of our whole systems on the NarrativeQA Book QA task. Table~\ref{tab:reader_model_performance} lists our results along with the state-of-the-art results reported in prior works (see Section \ref{ssec:baseline} and Fig.~\ref{fig:model_cheatsheet} for reference).
Empirically, our best ranker is from the combination of heuristic distant supervision and the unsupervised ICT training; our best reader is from the combination of the FiD model plus book prereading (with the top-10 ranked paragraphs as inputs). 
It is observed that specifically designed pre-training techniques play the most important role.
Details of the best ranker and reader can be found in the ablation study.


% Our best systems exceed the baselines on test set in both extractive and generative setting. 
Overall, we significantly raise the bar on NarrativeQA by 4.7\% over our best baseline and 6.8\% over the best published one.\footnote{Appendix \ref{app:append_full_results} reports the full results of our extensive experiments, where we achieve the best performance across all of the metrics.} But there is still massive room for future improvement, compared to the upperbound with oracle ranker.
Our baseline is better than all published results with simple BM25 retrieval, showing the importance of reader investigation.
Our best ranker (see Section~\ref{ssec:exp_ranker} for details) contributes to $2.5$\% of our improvement over the baseline. 
% Our best ranker (see Section~\ref{ssec:exp_ranker} for detailed model selection) contributes to 1.4\% in Rouge-L on extractive systems, and $2.5$\% on generative systems. 
% 
% Among all the generative reader models, BART outperforms GPT-2 and T5 by a notable margin. 
Our best reader (see Section~\ref{ssec:exp_reader} for details) brings an additional $>$2\% improvement compared to the BART reader. 
% Our book prereading techniques bring an additional $1$ point on dev set and $1.4$ points on test set to the best BART reader. Overall, we significantly raise the bar on NarrativeQA dataset, but there is still massive room for future improvement of both ranker and reader when compared to the performance with oracle ranker.

%%%%% significance test %%%%%%
We conduct a significance test for the results of our best system. There is no agreement on the best practice to validate the improvements~\cite{clark2011better,riezler2005some,dodge2019show} in the field of natural language processing.  We choose the non-parametric bootstrap test, because it is a more general approach and does not assume specific distributions over the samples. 
For bootstrapping, we sample 10K subsets, the size of each is 1K.
The small p-value (< 0.01) shows the effectiveness of our best model.



As a final note, even the results with oracle IR are far from perfect. It indicates the limitation of text-matching-based IR; and further confirms the challenge of evidence retrieval in Book QA.

%%%%% VERSION 2 %%%%%
% Table~\ref{tab:reader_model_performance} show that our best results exceed the original state-of-the-art methods for both generative and extractive models. Both families of models share some common trends: with the same reader, our distantly-supervised and unsupervised rankers all edge out the baseline BM25 ranker, among which the ORQA ranker is the most effective and stable. Our adaptation of the HARD EM training strategy shows improvement, but there is inconsistent improvement over different readers. With the same ranker, the BART reader has the best performance.

%%%%% VERSION 1 %%%%%
% Table~\ref{tab:reader_model_performance} and Table~\ref{tab:extractive_reader_model_performance} show that our best results exceed the original state-of-the-arts by $45\%$ and $30\%$ on test set for respectively generative and extractive models. Both tables also share some common trends. With the same reader, our distantly-supervised and unsupervised rankers all edge out the baseline BM25 ranker, among which the ORQA ranker is the most effective and stable one. Our adaptation of the HARD EM training strategy brings improvement, but the improvement over different readers is inconsistent. With the same ranker, the BART reader produces the best performance. 

% We note that BERT-heur~\cite{frermann-2019-extractive} uses the book summaries as strong supervision\footnote{Summaries have good coverage of true answers due to the data collection procedure, but it does not hold in general.} for evidence retrieval:
% Without using summaries that are regarded as unavailable in Book QA, we still achieve slightly better results, showing our ranker improvement techniques compensate for the lack of strong supervision.
% \footnote{Nearly 90\% of the true answers have a closely-alike expression in the summary due to the data collection procedures.}

%%%%% VERSION 1 %%%%%
% We achieve the new state-of-the-art with the usage of our distantly supervised BERT ranker and pre-trained LM-based readers. Specifically, our best combination can bring a consistent increase of 1 to 6 points across all metrics, compared to the previous state-of-the-art generative models. Similar improvements are also achieved in extractive QA task where our best combination of our BERT ranker and BERT extractive reader beats the previous state-of-the-arts and adds 1 to 4 points to most of the metrics. A special mention to BERT-heur~\cite{frermann-2019-extractive} in Table~\ref{tab:extractive_reader_model_performance} which takes the advantage of the corresponding summary in NarrativeQA as strong supervision\footnote{We find that nearly 90\% of the true answers have a closely-alike expression in the summary} for evidence retrieval. Note that the summary is unavailable in BookQA. Our outperformance on Rouge-L justifies the effectiveness of our distant supervision, compensating the deficiency of strong supervision signals in training.




% \begin{table}[t!]%[width=\textwidth]
%     \small
%     \centering
%     \setlength{\tabcolsep}{5pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1} % Default value: 1
%     \begin{tabular}{lcccccc} 
%         \toprule
%         \bf System & \multicolumn{2}{c}{\bf Rouge-L}\\
%         & \bf dev & \bf test \\
%         \midrule
%         \multicolumn{3}{c}{\bf Public Extractive Baselines}    \\
%         BiDAF~\cite{kovcisky2018narrativeqa}              & 6.33 & 6.22    \\
%         R$^3$ \cite{wang2018r} & 11.40 & 11.90 \\
%         \midrule
%         \multicolumn{3}{c}{\bf Our Extractive QA Models}\\
%         BM25 + BERT Reader (baseline)      & 12.59 & 13.81  \\
%         Our Ranker + BERT Reader            & \textbf{15.42} & 15.22  \\
%         \quad + book pre-reading \\
%         \quad + \it repl Ranker with Oracle &\textit{28.33} & \textit{28.72} \\
%         \midrule
%         \multicolumn{7}{c}{\bf Extractive Models w/ additional supervision}   \\
%         BERT-heur \cite{frermann-2019-extractive} & - & 15.15   \\
%         \midrule
%         \multicolumn{3}{c}{\bf Our Extractive QA Models (Ranker Analysis)}\\
%         BM25 + BERT Reader      & 12.59 & 13.81  \\
%         % \quad + BERT Ranker & 14.47/14.69 & \bf1.67/1.43   & \bf4.99/4.97 & \bf15.00/15.13 & \bf6.40/6.10 & \bf14.01/14.09 \\
%         \quad + BERT Ranker     & 14.76 & \textbf{15.49}  \\
%         \quad + HARD EM         & 14.10 & 14.42  \\
%         \quad + ORQA            & \textbf{15.42} & 15.22  \\
%         \quad + \it Oracle IR (BM25 w/ Q+A) & \textit{28.33} & \textit{28.72} \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-1mm}
%     \caption{\small{Extractive Book QA system performance (\%) on NarrativeQA full-story setting (Book QA setting). \textit{Oracle IR} combines question and true answers for retrieval. See Table~\ref{tab:extractive_reader_model_performance_full} in Appendix~\ref{sec:append_full_results} for the complete metrics.}}
%     \vspace*{-2mm}
%     \label{tab:extractive_reader_model_performance}
% \end{table}




\subsection{Ranker Ablation}
\label{ssec:exp_ranker}
To dive deeper into the effects of our ranker training techniques in Sec.~\ref{ssec:model_ranker}, we study the intermediate retrieval results and measure their coverage of the answers. The coverage is estimated on the top-5 selections of a ranker from the baseline BM25's top-32 outputs, by both the maximum Rouge-L score of all the overlapped subsequences of the same length as the answer in the retrieved passages; and a binary indicator of the appearance of the answer in the passages (EM). 

%%%%%  VERSION 2  %%%%%
% The ablation study in Table~\ref{tab:reader_model_performance} and~\ref{tab:extractive_reader_model_performance} shows that our ORQA ranker contributes 1 - 3.6 points Rouge-L improvement to the end-goal performance on test set for different readers. To dive deeper into the effect of our distant supervised and unsupervised techniques on evidence retrieval, we study the intermediate retrieval results and measure their coverage regarding to the answer. The coverage is estimated by both the maximum Rouge-L score of all the overlapped subsequences of the same length as the answer in the retrieval; and a binary indicator of the appearance of the answer in the retrievals (EM). 

%%%%%  VERSION 1  %%%%%
% The ablation study of our models in Table~\ref{tab:reader_model_performance} and~\ref{tab:extractive_reader_model_performance} shows that our distantly supervised BERT ranker contributes 1-2 points among the overall rise in all metrics. To dive deep into the effect of our distant supervision on evidence retrieval, we study the selection result and measure its coverage regarding to the answer. The coverage is estimated by both the maximum Rouge-L score of all the overlapped subsequences of the same length as the answer in the retrieval; and a boolean score indicating the appearance of the answer in the retrievals (EM). 

Table~\ref{tab:ir_model_performance} gives the ranker-only ablation. On one hand, our best ranker improves both metrics. It also significantly boosts the BART reader compared to the DS-ranker~\cite{mou2020frustratingly}, as shown in Appendix~\ref{app:append_full_results}.
On the other hand, on top of the DS ranker,  
% The performance drop caused by replacing BERT with BiDAF or MatchLSTM models further demonstrates the superiority of the pre-trained LM.
none of the other techniques can further improve the two ranker metrics significantly.
The ICT unsupervised training brings significant improvement over BM25. When adding to the DS-ranker, it brings slight improvement and leads to our best results.
Hard EM~\cite{min2019discrete} does not lead to improvements. Our conjecture is that generative readers does not solely generate purely matching-oriented signals, thus introduces noise in matching-oriented ranker training. 

The limited improvement and the low absolute performance demonstrate the difficulty of retrieval in Book QA. The gap between our best performance and the upper-bound implies that there is a large potential to design a more advanced ranker.

Additionally, we show that how much useful information our best ranker can provide to our readers in the whole QA system. 
In our implementation, the BART and FiD readers use top-3 and top-10 paragraphs from the ranker respectively.
The top-3 paragraphs from our best ranker give the answer coverage of 22.12\% EM and 49.83\% Rouge-L; and the top-10 paragraphs give 27.15\% EM and 56.77\% Rouge-L.
In comparison, the BM25 baseline has 15.75\%/43.44\% for top-3 and 24.08\%/53.55\% for top-10.
Therefore, our best ranker efficiently eases the limited-passage bottleneck brought by the ranker and benefits BART reader much more, which is consistent with our observations in Table~\ref{tab:reader_ablation}, Section~\ref{ssec:exp_reader}.

% The rest of the gain comes from the effective encoding and representation capability of BERT model. The performance drop caused by replacing BERT with BiDAF or MatchLSTM models demonstrates the superiority of the pre-trained LM. The observation matches the common trend in Table~\ref{fig:full_experiments} that our ORQA ranker contributes 1 - 3.6 points Rouge-L improvement to the end-goal performance on test set for different readers. On the other hand, the low absolute values of the metrics demonstrate the difficulty of the Book QA retrieval. The gap between our best performance and the upper-bound implies that there is large potential to design a more advanced ranker. 
% the mutual gaps among the baseline, our best model, the upper-bound and the oracle suggest the relatively limited progress we make and the potential of the future effort. They also implies the challenging aspect of the task that even with the state-of-the-art off-the-shelf models, we are not even close to being able to effectively extract the relevant information from the book context against the question.


% It aligns with the observation that Hard EM is more effective in extractive QA than in generative QA.

% \begin{table}[t!]
%     \small
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         \bf IR Method & \bf EM & \bf Rouge-L         \\
%         \midrule
%         BM25 &18.99 & 47.48 \\
%         BERT ranker (with ICT) & 21.29 & 50.35 \\
%         \textit{BERT ranker (with DS)}  & \it 24.26 & \it 52.68 \\
%         \quad \it - Rouge-L filtering & \it 22.63 &\it 51.02 \\
%         \quad + Hard EM & 22.45 & 50.50 \\
%         \quad + ICT pre-training$^*$  & \bf 24.83 & \bf 53.19 \\
%         \quad \it Repl BERT w/ BiDAF & \it 21.88 & \it 50.64 \\
%         \quad \it Repl BERT w/ MatchLSTM & \it 21.97 & \it 50.39 \\
%         \midrule
%         % Our Ranker (top-5) &  24.83 &  53.19 \\
%         BM 25 (top-3)$^{**}$ & 15.75 & 43.44\\
%         BM 25 (top-10)$^{***}$ & 24.08 &53.55\\
%         % BM 25 (top-16) & 26.85 &57.11\\
%         Our best ranker (top-3)$^{**}$ &  22.12 &49.83 \\
%         Our best ranker (top-10)$^{***}$ &  27.15 &  56.77 \\
%         % Our Ranker (top-16) &  29.00 &  59.03 \\
% %         |q-search-bm25|10|912.00/3359|27.15 |1906.89/3359|56.77|
% % |q-search-bm25|16|974.00/3359|29.00 |1982.88/3359|59.03|
%         \midrule
%         Upperbound (BM25 top-32) & 30.81 & 61.40\\
%         Oracle (BM25 w/ Q+A) & 35.75 & 63.92\\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-2mm}
%     \caption{\small{Ranker performance (top-5) on dev set. *: our best ranker used in Table \ref{tab:reader_model_performance}, which mimics the REALM training pipeline~\cite{guu2020realm} in the Book QA setting. In the middle block we list top-3/10 results, which are used in our readers (** for BART and *** for FiD, see our reader ablation in Section~\ref{ssec:exp_reader}). Results in \textit{italic} are achieved with the methods from \cite{mou2020frustratingly}.
%     % All the values are averaged over dev samples.
%     }}
%     \vspace*{-3mm}
%     \label{tab:ir_model_performance}
% \end{table}

\begin{table}[t!]
    \small
    \centering
    \setlength{\tabcolsep}{4pt} % Default value: 6pt
    \begin{tabular}{lcc}
        \toprule
        \bf IR Method & \bf EM & \bf Rouge-L         \\
        \midrule
        \multicolumn{3}{c}{\bf Baseline Rankers}    \\
        BM25                        & 18.99 & 47.48 \\
        % BM25 (top-3 for BART)       & 15.75 & 43.44\\
        % {\color{red} \it BM25 (top-10 for FiD) }      & \it 24.08 & \it 53.55 \\
        BERT DS-ranker~\cite{mou2020frustratingly}              
                                    & 24.26 & 52.68 \\
        \quad - Rouge-L filtering   & 22.63 & 51.02 \\
        \quad Repl BERT w/ BiDAF    & 21.88 & 50.64 \\
        \quad Repl BERT w/ MatchLSTM & 21.97 & 50.39 \\
        
        \midrule
        \multicolumn{3}{c}{\bf Our Rankers}    \\
        BERT ICT-ranker             & 21.29 & 50.35 \\
        BERT DS-ranker              \\
        \quad + Hard EM             & 22.45 & 50.50 \\
        \quad + ICT pre-training$^*$  & \bf 24.83 & \bf 53.19 \\
    %     Our best ranker$^*$ (top-3 for BART)  & 22.12 & 49.83 \\
    %   {\color{red} \it Our best ranker$^*$ (top-10 for FiD)}  & \it 27.15 & \it 56.77 \\
        
        \midrule
        \multicolumn{3}{c}{{\bf Oracle Conditions} }    \\
        Upperbound (BM25 top-32) & 30.81 & 61.40\\
        Oracle (BM25 w/ Q+A) & 35.75 & 63.92\\
        \bottomrule
    \end{tabular}
    \vspace*{-2mm}
    \caption{\small{Ranker performance (top-5) on dev set. Asterisk (*) indicates our best ranker used in Table \ref{tab:reader_model_performance}.
    % , which mimics the REALM training pipeline~\cite{guu2020realm} in the Book QA setting. 
    % We also list top-3/10 results which are used in our BART/FiD readers in Section~\ref{ssec:exp_reader}.
    % {\color{red} Top-10 results are not directly comparable to other results and are provided for exposition only.}
    }}
    \vspace*{-3mm}
    \label{tab:ir_model_performance}
\end{table}



\subsection{Reader Ablation}
\label{ssec:exp_reader}

\begin{table}[t!]%[width=\textwidth]
    \small
    \centering
    \setlength{\tabcolsep}{5pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1} % Default value: 1
    \begin{tabular}{lcccccc} 
        \toprule
        \multirow{2}{*}{\bf System} & \multicolumn{2}{c}{\bf Rouge-L}\\
         & \bf dev & \bf test \\ 
        \midrule
        BM25 + BART reader (baseline)       & 23.16     & 24.47     \\
        \quad + BART-FiD reader             & 25.95     & --        \\
        Our ranker + BART reader            & 25.83     & 26.95     \\
        \quad + BART-FiD reader             & 26.27     & --        \\
        \quad repl BART w/ GPT-2            & 22.22     & --    \\%& 22.95 \\
        \quad repl BART w/ T5               & 20.57     & --    \\%& 21.22 \\ 
        \quad + book preread                & 26.82     & --    \\%& 28.31 \\
        \quad \quad + BART-FiD Reader$^*$   & \bf 27.91 & \bf 29.21 \\
        \quad + book preread (\emph{decoder-only})  & 26.51     & --\\ 
        \bottomrule
    \end{tabular}
    \vspace*{-2mm}
    \caption{\small{Ablation of our Reader Model. Asterisk (*) indicates our best reader used in Table \ref{tab:reader_model_performance}.}}
    \vspace*{-4mm}
    \label{tab:reader_ablation}
\end{table}

% Based on Chenghao's results
% \begin{table}[t!]%[width=\textwidth]
%     \small
%     \centering
%     \setlength{\tabcolsep}{5pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1} % Default value: 1
%     \begin{tabular}{lcccccc} 
%         \toprule
%         \multirow{2}{*}{\bf System} & \multicolumn{2}{c}{\bf Rouge-L}\\
%          & \bf dev & \bf test \\ 
%         \midrule
%         BM25 + BART reader (baseline)       & 23.16     & 24.47     \\
%         % \quad + BART-FiD Reader (top-1) & 20.22 & - \\
%         % \quad + BART-FiD Reader (top-8) & 24.68 & - \\
%         \quad + BART-FiD reader & 25.11& -- \\
%         % \quad + BART-FiD Reader (top-16) & 25.88& - \\
%         Our ranker + BART reader            & 25.83    & 26.95$^\dagger$     \\ 
%         % \quad + BART-FiD Reader (top-1) &  & - \\
%         % \quad + BART-FiD Reader (top-8) &  & - \\
%         \quad + BART-FiD reader & 25.24& -- \\
%         % \quad + BART-FiD Reader (top-16) & 25.50 & - \\
% % {
% %     "Bleu_1": 0.2503156661040933,
% %     "Bleu_2": 0.07730978058124241,
% %     "Bleu_3": 0.02530519412474822,
% %     "Bleu_4": 0.00808357619271654,
% %     "METEOR": 0.16477000283127768,
% %     "ROUGE_L": 0.2525213551469742,
% %     "CIDEr": 0.0
% % }
%         \quad + book preread$^*$     & \bf 26.82 & \bf 28.31$^\dagger$ \\
%         \quad \quad + BART-FiD Reader & 25.58 & -- \\
%         \quad + book preread (\emph{decoder-only})            & {26.51}     & --\\ % \textcolor{red}{27.27}      \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-2mm}
%     \caption{\small{Ablation of our Reader Model. *: our reader used in the best full system in Table \ref{tab:reader_model_performance}.}}
%     \vspace*{-4mm}
%     \label{tab:reader_ablation}
% \end{table}

Table~\ref{tab:reader_ablation} shows how the different reader techniques in Section~\ref{ssec:model_reader} contribute to the QA performance.

First, switching the BART reader to FiD gives a large improvement when using the BM25 ranker (2.8\%), approaching the result of ``our ranker + BART''.
This agrees with our hypothesis in Section~\ref{ssec:model_reader} Analysis 2, that FiD takes the roles of both ranker and reader.
% 
Second, although the above result shows that FiD's ranking ability does not add much to our best ranker, our cross-paragraph attention enhancement still improves FiD due to better retrieval results (0.5\% improvement over ``our ranker + BART'').
% 
Third, among all the generative reader models, BART outperforms GPT-2 and T5 by a notable margin. 
Finally, the book prereading brings consistent improvements to both combinations; and the combination of our orthogonal reader improvements finally gives the best results. We also confirm that the prereading helps decoders mostly, as only training the decoder gives comparable results.

% with chenghao's results
% Table~\ref{tab:reader_ablation} shows how the different reader techniques in Section~\ref{ssec:model_reader} contribute to the QA performance.
% First, when the baseline BM25 retriever is used, we observe $\sim$2\% improvement from switching the BART reader to the FiD reader. However, FiD does not help when our improved ranker is used. This agrees with our hypothesis in Section~\ref{ssec:model_reader} Analysis 2, that FiD helps via integrating the jobs of both ranker and reader. However, FiD's ranking ability does not add much to our best ranker. In the meanwhile, with the shorter inputs provided by our ranker, the BART encoder is able to capture the interactions among paragraphs via their concatenation. This explains the slightly better (0.6\%) result of BART reader over our top-3 paragraphs, versus the FiD reader over our top-10 results.

% On the other hand, the book prereading technique improves the reader in an orthogonal way to the ranker. It enables a further 1\% improvement, which corresponds to our best reader model. Also, the prereading helps most in decoders, as training the decoder only gives comparable results.

% \begin{table}[t!]%[width=\textwidth]
% \setlength{\tabcolsep}{4pt}
%     \small
%     \centering
%     \begin{tabular}{lcccccc} 
%         \toprule
%         \bf System & \multicolumn{2}{c}{\bf Rouge-L}\\
%         & \bf dev & \bf test \\
%         \midrule
%         \multicolumn{3}{c}{\bf Extractive Readers}    \\
%         % BiDAF~\cite{kovcisky2018narrativeqa}               & 33.45/33.72 & 15.69/15.53 & 15.68/15.38 & 36.74/36.30\\
%         BERT + Hard EM~\cite{min2019discrete} & \bf 58.1 & \bf 58.8   \\
%         BERT-only~\cite{min2019discrete}      & 55.8 & 56.1       \\
%         % BERT-heur \cite{frermann-2019-extractive} & -/\bf50.36 & -/24.24 & -/\bf27.09 & -/58.50\\
%         % \midrule
%         % \multicolumn{5}{c}{\bf Our Extractive Readers}               \\
%         BERT w/ full training signals [\textbf{ours}] & 52.62 & 52.02    \\
%         BERT w/ clean signals only$^{*}$ [\textbf{ours}] & 57.19 & 56.35  \\
%         % BERT w/ exact answer match only &  51.33 & 39.05 & 26.84 & 57.32/&32.25&48.94 \\bf   \\\
%         \midrule
%         \multicolumn{3}{c}{\bf Generative Readers}    \\
%         % Attention Sum~\cite{kovcisky2018narrativeqa} & 23.28 & 22.26   \\
%         Masque~\cite{nishida2019multi} & - & 54.74  \\
%         % GPT-2
%         % GPT-2 Reader [\textbf{ours}] & 34.32 & 35.65  \\
%         % BART
%         BART Reader [\textbf{ours}] & \textbf{60.46} & \textbf{58.76}  \\
%         % T5
%         % T5 Reader [\textbf{ours}] & 53.61 & 54.28  \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-1mm}
%     \caption{\small{Reader performance under NarrativeQA summary setting (\%). *Clean signals refer to the label spans by exact answer match. We compare with the best public extractive model from~\cite{min2019discrete} and its BERT-only ablation; and the best generative model from~\cite{nishida2019multi}. }
%     }
%     \vspace*{-2mm}
%     \label{tab:reader_performance_on_summary}
% \end{table}

% \paragraph{Reader-Only Evaluation}
% Finally, we confirm that our enhancements are based on existing state-of-the-art reader models, so that the improvement we achieve is advancing the new state-of-the-art of the Book QA field. To eliminate the effects of the ranker, we inspect the modeling capability of different readers in the \emph{summary setting} of NarrativeQA. As confirmed by Table~\ref{tab:reader_performance_on_summary}, our best BERT extractive model and the BART generative model both attain state-of-the-art and have close performance. 

% Firstly, this confirms that the readers we use in our Book QA system are state-of-the-arts. Secondly, the two readers have large performance gap on the Book QA setting, showing the fundamental differences between the Book QA and the summary setting. 
% Finally, another interesting finding is that GPT-2 does not work as well as the other methods, but with our training objective from Eq. (\ref{eq:reader_input}) the gap becomes very small on the Book QA setting. We hypothesize it is because our training objective that includes context prediction could enhance the decoding of narrative phrases/sentences, which might be an interesting direction for future study.

% Table~\ref{tab:reader_model_performance} and~\ref{tab:extractive_reader_model_performance} have proved the efficacy of pre-trained LM readers on the BookQA task. Here we conduct another set of experiments on NarrativeQA summary settings where summaries are provided and used as evidence, to inspect the modeling capability of different readers without the disturbance from rankers. 

% As shown in Table~\ref{tab:reader_performance_on_summary}, our best BERT extractive model is slightly better on test set than the BERT-only method with cleaned training data in \cite{min2019discrete}, but worse than their BERT with Hard EM. However, we are not able to reproduce the obvious gain in BookQA using our BERT with Hard EM, justified by the similiar findings in open-domain QA from \cite{min2019discrete, cheng2020probabilistic}.

% For generative models, we observe the great help from pre-trained LMs and our unsupervised training techniques, as well as the potential application of pointer generator(PG) in BookQA based on the remarkable gain obtained in \cite{tay2019simple}. \cite{nishida2019multi} deeply integrates the PG structure into transformer blocks~\cite{vaswani2017attention} and reaches the previous state-of-the-art, stressing the importance of PG in generative QA task. Considering the claim made in \cite{tay2019simple} about the limited contribution of PG under NarrativeQA full-story setting through their ablation study, we attribute the gain from \cite{nishida2019multi} to the deep integration of the PG with the transformer block.

%%%%%  VERSION 1  %%%%%
% Table~\ref{tab:reader_model_performance} and~\ref{tab:extractive_reader_model_performance} have proved the efficacy of pre-train LM readers on the BookQA task. But the interest in knowing better about its features independently from the ranker drives us to conduct another set of experiments on NarrativeQA summary settings where summaries are provided and used as evidence.

% As shown in Table~\ref{tab:reader_performance_on_summary}, our BERT extractive model is slightly better on test set than the BERT-only method with cleaned training data in \cite{min2019discrete}, but worse than their BERT with Hard EM. However, we are not able to reproduce the obvious gain in BookQA using our BERT with Hard EM, justified by the similiar findings in open-domain QA from \cite{min2019discrete, cheng2020probabilistic}. For generative models, we observe the great help from pre-trained LMs and potential application of pointer generator in BookQA based on the remarkable gain obtained in \cite{tay2019simple}. 

% \cite{nishida2019multi} deeply integrates the pointer generator structure into transformer blocks and reaches the state-of-the-art, stressing the importance of pointer generator in generative QA task. Considering the claim made in \cite{tay2019simple} about the limited contribution under NarrativeQA full-story setting through their ablation study, we attribute the gain from \cite{nishida2019multi} to the deep integration of the pointer generator with the transformer block which is the basic unit structur in the most prevailing LMs.







% \begin{figure*}[h!]
%     \fontsize{8}{10.5}\selectfont
%     \centering
%     \begin{tabular}{lcp{5.9cm}p{5.8cm}}
%     % \begin{tabular}{lp{10cm}p{7cm}}
%         \toprule
%         \textbf{Evidence Type} & \textbf{Sub Type} & \textbf{Description} & \textbf{Example}         \\
%         \midrule
%         \multirow{7}{*}{Concept}    
        
%         & \multirow{3}{*}{Entity}     
%         & {Standard named entities like person, location and organization names. Book-specific character names and their co-references are also included.} 
%         & \multirow{3}{5.6cm}{\textbf{Q}: What is the name of \underline{Mortimer Treginnis}' sister? \textbf{A}: \underline{Brenda}} \\ 
        
%         & Common Noun- 
%         & \multirow{2}{5.6cm}{Common nouns or noun phrases that are universally used across books and other literature} 
%         & \multirow{2}{5.6cm}{\textbf{Q}: What was Rodgers exposed to while investigating? \textbf{A}: \underline{Radioactive gas}}      \\
        
%         &Phrases&&  \\
        
%         & \multirow{2}{*}{Book-Specific} 
%         & \multicolumn{1}{p{5.6cm}}{Common nouns or noun phrases that have special meanings or importance in the book of interests}  
%         & {\textbf{Q}: Where do Anne and Philippa stay after their first year in college? \textbf{A}: \underline{Patty's place}}   \\
        
%         \midrule
        
%         \multirow{4}{*}{Event}      
%         & \multirow{2}{*}{Event Expression}    
%         & {Standard textual expression of event structures about "\emph{who did what to whom, when, where and how}"} 
%         & \multirow{2}{6cm}{\textbf{Q}: In what way did \underline{Christopher atone for his sin}? \textbf{A}: \underline{He helped Will escape and accepted the punishment}} \\ 
%         & \multirow{2}{*}{Event Name}  
%         & \multicolumn{1}{p{5.6cm}}{Sometimes an important or famous event will be referred with a name} 
%         & {\textbf{Q}: When did Harney and Charity kiss for the first time? \textbf{A}: On \underline{the trip to Nettleton}}    \\
        
%         \midrule
        
%         \multirow{8}{*}{Attribute}  
%         & \multirow{2}{*}{States}     
%         & \multicolumn{1}{p{5.6cm}}{The textual description of the state of an entity or concept as an attribute} 
%         & {\textbf{Q}: Why does the princess agree to let Ermyntrude pretend to be her? \textbf{A}: Because she is \underline{timid}} \\ 
        
%         & \multirow{2}{*}{Numerics} & \multirow{2}{5.6cm}{Standard attributes with numeric values}  
%         & {\textbf{Q}: How may volumes has Darnley written on the origins of life? \textbf{A}: \underline{Three}} \\
%         % & \multirow{2}{*}{Descriptions} & \multicolumn{1}{p{5.6cm}}{An attribute of an entity or concept which does not have a short attribute phrase to summarize} & {\textbf{Q}: What does Beerbohm say is the one habit that makes Soames noticable? \textbf{A}: \underline{He always wears} \underline{the same gray cape and soft black hat}} \\
        
%         & \multirow{2}{*}{Descriptions} 
%         & \multicolumn{1}{p{5.6cm}}{An attribute of an entity or concept which does not have a short attribute phrase to summarize} 
%         & \multirow{2}{5.8cm}{\textbf{Q}: Why didn't Anne accept Gilberts proposal? \textbf{A}: \underline{She's dreaming of true love}} \\
        
%         & \multirow{2}{*}{Book Attributes} 
%         &         \multirow{2}{*}{Attributes of books themselves, like theme etc.}
%         & {\textbf{Q}: Name the major theme used in the Adventures of Sherlock Holmes? \textbf{A}: \underline{Social injustice}} \\
%         \bottomrule
%     \end{tabular}
%     % \vspace*{-2mm}
%     \caption{\small{The definitions of the evidence types.}}
%     % \vspace*{-2mm}
%     \label{fig:semantic_unit_definition}
% \end{figure*}
% % }
% % \endgroup


==> model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
%%%%%%%%%%%%%  Proposed Method  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[ht!]
%     \includegraphics[width=\textwidth]{imgs/system.png}
%     \centering
%     \caption{System architecture with distant training. The dotted line indicates that the data flow is optional. }
%     \label{fig:system_architecture}
% \end{figure*}

\begin{figure*}[ht!]%[width=\textwidth]
    \small
    \fontsize{6.5}{10.5}\selectfont
    \centering
    \begin{tabular}{C{0.11\textwidth}
            C{0.17\textwidth}
            C{0.35\textwidth}
            C{0.29\textwidth}}
        \toprule
        \textbf{Target Module} &\textbf{Approach} & \textbf{Original Idea in ODQA} & \textbf{Our Improved Version for Book QA}   \\
        \midrule
        \multirow{4}{*}{Reader} &  \multirow{2}{*}{Book Prereading}&  \citet{sun2019improving} adapt GPT on general QA datasets;  \citet{xiong2019pretrained} adapt BERT on Wikipedia as entity prediction. & We propose to adapt BART to the narrative style with the text-infilling objective. \\
        % \textcolor{blue}{BiDAF} \cite{kovcisky2018narrativeqa} & &\\
        \cdashline{2-4}
        & \multirow{2}{*}{Fusion-in-Decoder}& Proposed by \cite{izacard2020leveraging} as a new type of ODQA reader. &  We improve the decoder with attention over all the encoder states to capture cross-passage interaction. \\
        \midrule
        \multirow{4}{*}{Ranker} & \multirow{1}{*}{Heuristic distant supervision} &  \multirow{1}{*}{N/A} & N/A$^*$ \\
        \cdashline{2-4}
        & \multirow{2}{*}{Unsupervised ICT} & Proposed by \cite{Lee_2019orqa} as siamese network for both BERT pre-training and dense retrieval. & We improve the method with our book-specific training data selection. \\
        \cdashline{2-4}
        &Hard EM & Proposed by \cite{min2019discrete} for reader training. & We adapt the method for ranker training. \\
        \bottomrule
    \end{tabular}
    \vspace*{-2mm}
    \caption{{Summary of our inspected approaches in Analysis Part I. *We directly apply the heuristics from~\cite{mou2020frustratingly} for Book QA.}}
    \vspace*{-3mm}
    \label{fig:analysis_cheatsheet}
\end{figure*}

% \section{Analysis Part I: How State-of-the-Art Open-Domain QA Techniques Help}
\section{Analysis Part I: Experimental Study}
This section describes our efforts of applying or adapting the latest open-domain QA ideas to improve Book QA ranker/reader models.
Fig.~\ref{fig:analysis_cheatsheet} summarizes our inspected approaches.
The experimental results quantify the challenges in Book QA beyond open-domain QA.

 

% In this section, we discuss from both the ranker and reader perspectives about the usage of the baseline models and our effort of applying the latest ODQA techniques to Book QA as motivated in Sec.\ref{sec:introduction}.

%%%%% Version 1 %%%%%
% In this section, we will first define the task of Book QA. Then we will introduce the modules of our system and describe the details about fine-tuning the pre-trained LM-based models for the Book QA task. Our model architecture is adapted from ODQA as motivated in Sec.\ref{sec:related_word_bookqa}.

% Practically, in most cases, not all such paragraphs need to be considered \cite{kovcisky2018narrativeqa}. We can first utilize a light-weight \textbf{ranker model} to filter out a candidate paragraph set $\filteredContextSet$ (``evidence'') as a proxy to $\contextSet$ and then only run computationally expensive \textbf{reader  model} on $\filteredContextSet$. This idea naturally gives rise to the idea of the classic \textbf{ranker-reader} solution of the open-domain QA system. 





\subsection{QA Reader}     \label{ssec:model_reader}

\paragraph{Base Reader Models}
We study the usage of different pre-trained LMs on Book QA, including BART~\cite{lewis2019bart}, GPT-2~\cite{radford2019language}, T5~\cite{raffel2019exploring} and BERT~\cite{devlin2018bert}.
The first three are \emph{generative} readers and can be directly trained with the free-form answers as supervision. 
Specifically, during training we treat $\question \oplus \text{[SEP]} \oplus \filteredContextSet[\question]$ as input to generate answer $\realAnswer$, where $\text{[SEP]}$ is the special separation token and $\oplus$ is the concatenation operator.

For the \emph{extractive} reader (BERT), we predict the most likely span in $\filteredContextSet[\question]$ given the concatenation of the question and the evidence $\question \oplus \text{[SEP]} \oplus \filteredContextSet[\question]$.
Due to the generative nature of Book QA, the true answer may not have an exact match in the context. Therefore, we follow~\citet{mou2020frustratingly} to find the span $\mathbf{S}$ that has the maximum Rouge-L score with the ground truth $\realAnswer$ as the weak label, subject to that $\realAnswer$ and $\mathbf{S}$ have the same length (i.e. $|\mathbf{S}|=|\realAnswer|$).

% We fine-tune a BERT model pre-trained on SQuAD~\cite{Rajpurkar_2018squad} to predict the most likely span in $\filteredContextSet[\question]$ given the question $\question$ and the evidence $\filteredContextSet[\question]$. We use the exact-answer spans as the gold labels for the training. However, they can be hardly found in the context due to the free-form nature of the true answer. To better supervise the training of the extractive BERT reader, we create sentence-level weak span annotations for each question instead. Specifically, we compute the Rouge-L score \cite{lin-2004-rouge} between the true answer $\realAnswer$ and each candidate span $\mathbf{S}$ of the same length in the context (i.e. $|\mathbf{S}|=|\realAnswer|$), and finally take the span with the maximum Rouge-L score as our weak labels.

%%%%%  VERISION 1  %%%%%
% We fine-tune another BERT model pre-trained on SQuAD~\cite{Rajpurkar_2018squad}, an extraction-based QA dataset, to predict the most likely span of the answer given the question and the provided evidence following Eq~\ref{eq:extrative_model}.
% \begin{align} \label{eq:extrative_model}
%     P_{\text{start}}(w_i) &=
%     BERT(\vv{\filteredContextSet}, \vv{\question}) 
%     \\
%     P_{\text{end}}(w_i) &=
%     BERT(\vv{\filteredContextSet}, \vv{\question})
% \end{align}
% where $P_{\text{start}}(w_i)$ and $P_{\text{end}}(w_i)$ are the probability of being the starting and ending position for $i$-th token.

% The exact-answer spans are seen as the gold labels for the training. However, they can be hardly found in the context due to the free-form nature of the true answer. To better supervise the training of the BERT reader, we create sentence-level weak span annotation for each question instead. Specifically, we compute the Rouge-L score \cite{lin-2004-rouge} between the true answer and each candidate span of the same length in the context, and finally take the span with the maximum Rouge-L score as our weak labels.
% \begin{align} \label{eq:extractive_reader_label}
%     \text{span\_start} &= 
%     \argmax_n  
%     f( \{w_i\}_n^{n+|\realAnswer|},  \realAnswer )
%     \\
%     \text{span\_end} &= 
%     \text{start\_span} + |\realAnswer|
% \end{align}
% where $\{w_i\}_n^{n+|\realAnswer|}$ represents a subsequence starting from $n$-th to ($n+|\realAnswer|$)-th token; $f$ is the function to measure the similarity between each subsequence and the true answer, and $f(\cdot, \cdot) = \text{Rouge-L}(\cdot, \cdot)$ in our case.



% \paragraph{Base Reader Model (Generative)}
% For \emph{generative} reader, we use the BART~\cite{lewis2019bart}, GPT-2~\cite{radford2019language},  and T5~\cite{raffel2019exploring} models. 
% These autoregressive models are directly trained with the free-form answers as supervision. 
% We treat $\question \oplus \text{[SEP]} \oplus \filteredContextSet[\question]$ as input to generate answer $\realAnswer$.
% Following the recommended settings, we select $\mathbf{O}_1$ as autoregressive labels for GPT-2 and $\mathbf{O}_2$ for BART and T5, i.e.
% \par \vspace{-5mm}
% {\small
%     \begin{align} \label{eq:reader_input}
%         \mathbf{O}_1
%         &=  
%         \question \oplus \text{[SEP]} \oplus \filteredContextSet[\question]
%         \oplus
%         \text{[SEP]} \oplus \realAnswer,  \\
%         \mathbf{O}_2
%         &=  
%         \realAnswer.
%     \end{align}
% }%
% where $\oplus$ is the concatenation operator, and $\text{[SEP]}$ is a special separation token.

%%%%%  VERSION 2  %%%%%
% By design, GPT-2, BART and T5 are all autoregressive models and therefore do not require additional annotations for training. 
% Following their recommendations, we construct $\mathbf{O}_1$ as the autoregressive labels for GPT-2 and $\mathbf{O}_2$ for both BART and T5:
% \vspace*{-4mm}
% \begin{align} \label{eq:reader_input}
%     \mathbf{O}_1
%     &=  
%     \question
%     \oplus
%     \text{[SEP]}
%     \oplus
%     \filteredContextSet[\question]
%     \oplus
%     \text{[SEP]}
%     \oplus
%     \realAnswer,  \\
%     \mathbf{O}_2
%     &=  
%     \realAnswer.
% \end{align}
% where $\oplus$ is the concatenation operator, and $\text{[SEP]}$ is a special token.

%%%%%  VERISION 1  %%%%%
% We try GPT-2~\cite{radford2019language}, BART~\cite{lewis2019bart} and T5~\cite{raffel2019exploring} pre-trianed LMs for answer generation. By design, GPT-2, BART and T5 are all autoregressive models and therefore do not require additional annotations for training. During training and inference, we construct the initial input context $\mathcal{I}_0$ to both models by concatenating the question $\question$, a special separation token $\mathbf{SEP}$ and the given evidence $\filteredContextSet$ as shown in Eq~\ref{eq:reader_input}:
% \begin{align} \label{eq:reader_input}
%     \mathcal{I}_0 &= [ 
%         \question;
%         \mathbf{SEP}; 
%         \filteredContextSet[\question];
%         \mathbf{SEP}
%         ]
% \end{align}
% where ``;" is a concatenation operation, and $\question$, $\mathbf{SEP}$, $\filteredContextSet$ represent the corresponding tokens.

% GPT-2 only stacks transformer decoder blocks, hence its iterative generation procedure can be modelled by Eq~\ref{eq:gpt2_generation1} and Eq~\ref{eq:gpt2_generation2}.
% \begin{align} 
%     \label{eq:gpt2_generation1}
%     \mathcal{I}_{n} &= [ 
%         \mathcal{I}_{n-1};
%         \{y_i\}_0^{n-1}
%         ]
%     \\
%     \label{eq:gpt2_generation2}
%     y_n &= 
%     \text{decoder}(\mathcal{I}_n)
% \end{align}
% where $\{y_i\}_1^{n-1}$ represents the preceding tokens before the $n$-th in the prediction with $\{y_0\}$ denoting the starting token of each sentence.

% On the other hand, both BART and T5 take an extra step of encoding the input, i.e Eq~\ref{eq:bart_generation1}, and feed the output of the encoder into the decoder together with all preceding outputs of the decoder as shown in~\ref{eq:bart_generation2}.
% \begin{align} 
%     \label{eq:bart_generation1}
%     \vv{T} &=
%     \text{encoder} (\mathcal{I}_n)
%     \\
%     \label{eq:bart_generation2}
%     y_n &= 
%     \text{decoder} ( \vv{T}, \mathcal{I}_n )
% \end{align}
% where $\vv{T}$ is the contextual vector carrying the information from selected evidence and the existing generated answers.

\paragraph{Method 1: Book Prereading}
Inspired by the literature on the unsupervised adaptation of pre-trained LMs~\cite{sun2019improving,xiong2019pretrained}, we let the reader ``\textbf{preread}'' the training books through an additional pre-training step prior to fine-tuning with QA task.
This technique helps to better adapt to the narrative writing styles.
% Two \textbf{preread} techniques are investigated and compared on BART in terms of the end-goal performance.

% (1) We only pre-train the decoder with language modeling task using questions-specific paragraphs. We use $Q + \filteredContextSet[\question]$ as the decoder input and the autoregressive labels with the intention to encourage the decoder to familiarize the narrative language. During pre-training, we freeze the encoder parameters and replace its output with an all-zero vector. 

Specifically, we extract random passages from all training books to build a passage pool.
For each training iteration, we mask random spans from each passage, following the setting in~\cite{lewis2019bart}. The start positions of spans are sampled from a uniform distribution without overlapping. The length of each span is drawn from a Poisson distribution with $\lambda\!=\!3$. Each span is then replaced by a single \texttt{[mask]} token regardless of the span length. We mask $15\%$ of the total tokens in each passage. During the prereading stage, we use the masked passage as the encoder input and the raw passage as the decoder output to restore the raw passage in the auto-regressive way.
% (2) Prior to fine-tuning with QA task, we further adapt the base BART model to Narrative QA domain using text infilling task. We randomly extract passages from each book (train set only) to build a passage pool and mask them following the method in \cite{lewis2019bart}. The candidate spans in each passage are sampled from a uniform distribution without overlapping. The length of each span is drawn from a Poisson distribution with $\lambda=3$. Each span is then replaced by a single \texttt{[mask]} token regardless of the span length. We only mask $15\%$ of the total tokens in each passage. During re-pre-training, we use the masked passage as the encoder input and the raw passage as the decoder input to restore the raw passage in the auto-regressive way. 

\paragraph{Method 2: Fusion-in-Decoder}
Recently~\citet{izacard2020leveraging} scale BART reader up to large number of input paragraphs. The method, \textbf{Fusion-in-Decoder (FiD)}, first concatenates each paragraph to the question to obtain a question-aware encoded vector, then merges these vectors from all paragraphs and feeds them to a decoder for answer prediction. 
FiD reduces the memory and time costs for encoding the concatenation of all paragraphs, and improves on multiple ODQA datasets.
% 
FiD is an interesting alternative for Book QA, since it can be viewed as an integration of the ranker and reader, with the ranker absorbed in the separated paragraph encoding step. 

FiD trades cross-paragraph interactions for encoding more paragraphs. The single encoded vector per passage works well for extractive ODQA because the vector only needs to encode information of candidate answers. However, in Book QA, the answers may not be inferred from a single paragraph and integration of multiple paragraphs is necessary.
Therefore, in our approach, we concatenate the encoded vectors of all the paragraphs, and rely on the decoder's attention over these vectors to capture the cross-paragraph interactions. 

% Since there is no passage-level annotations in Book QA, FiD provides an alternative solution to ranker training.

% Recently~\cite{izacard2020leveraging} scale BART reader up to handle larger number of input paragraphs. The method, named \textbf{Fusion-in-Decoder (FiD)} reader, first concatenates each passage to the question to achieve question-aware encoding, then merges the encoded vectors for all passages and feeds them to a decoder for answer prediction. In this way it avoids the memory and time costs for encoding the concatenation of all passages, and improves on multiple open-domain QA datasets.

% We consider the FiD reader an interesting technique for Book QA, because the design of FiD can be viewed as an end-to-end model of the ranker-reader framework, with the ranker part absorbed in the separated passage encoding step. Since there is no passage-level annotations in Book QA, FiD provides an alternative solution to ranker training.


\subsection{Passage Ranker}     \label{ssec:model_ranker}

\paragraph{Base Ranker Model}
Our ranker is a BERT-based binary classifier fine-tuned for evidence retrieval. It estimates the likelihood of each passage to be supporting evidence given a question $\question$.
% It is supposed to estimate how likely each paragraph to be a supporting evidence in terms of the given question $\question$, i.e.:
% \begin{equation}
%     P(\passage) = BERT(\vv{\passage}, \vv{\question})
% \end{equation}
% where $\vv{\cdot}$ denotes the corresponding vector representation.

Training the ranker models is difficult without high-quality supervision.
To deal with this problem, we investigate three approaches for creating pseudo labels, including \emph{distant supervision, unsupervised ranker training and Hard EM training}.
% prepare a set of training data on NarrativeQA with pseudo labels created as follows. 

\paragraph{Method 1: Distant Supervision (DS)}
This is the baseline approach from~\cite{mou2020frustratingly}. It constructs DS signals for rankers in two steps: First, for each question $\question$, two BM25 rankers are used to retrieve passages, one with $\question$ as query and the other with both $\question$ and the true answer $\realAnswer$. Denoting the corresponding retrieval results as $\filteredContextSet[\question]$\footnote{For simplicity, we use the notation $\filteredContextSet[\question]$ here.} and $\filteredContextSet[\question + \realAnswer]$, the method samples the positive samples $\filteredContextSet[\question]^+$ from $\filteredContextSet[\question] \cap \filteredContextSet[\question + \realAnswer]$ and the negative samples $\filteredContextSet[\question]^-$ from the rest, with the ratio $\sigma \equiv |\filteredContextSet[\question]^+| / |\filteredContextSet[\question]^-|$ for each question $\question$ as a hyperparameter.
% \vspace*{-2mm}
% \begin{equation}
%     % \sigma = 
%     % \frac{|\filteredContextSet[\question]^+|}{|\filteredContextSet[\question]^-|}
%     \sigma \equiv |\filteredContextSet[\question]^+| / |\filteredContextSet[\question]^-|.
% \end{equation}
% where $\sigma$ is a hyperparameter.

% \begin{figure}[t!]
%     \includegraphics[width=0.4\textwidth]{imgs/data_sampling.png}
%     \centering
%     \vspace*{-2mm}
%     \caption{Data sampling for the ranker training}
%     \label{fig:system_architecture}
% \end{figure}

Second, to enlarge the margin between the positive and negative samples, the method applies a \textbf{Rouge-L filter} upon the previous sampling results to get the refined samples, $\mathcal{C}_\mathbf{Q}^{++}$ and $\mathcal{C}_\mathbf{Q}^{--}$:
% and only selects the samples whose answer-based Rouge-L score is higher or lower than the threshold. Denoting the new positive and negative samples as $\mathcal{C}_\mathbf{Q}^{++}$ and $\mathcal{C}_\mathbf{Q}^{--}$, they should follow Eq~\ref{eq:positive_samples} and Eq~\ref{eq:negative_samples}:
\par 
\vspace*{-5mm}
{\small
    \begin{align}
    % \vspace*{-2mm}
        % \label{eq:positive_samples}
        % \filteredContextSet[\question]^{++} = 
        % \filteredContextSet[\question]^+
        % \cap
        % \{\passage|Rouge\text{-}L(\passage, \realAnswer)>\alpha\} 
        % \\
        \filteredContextSet[\question]^{++} = 
        \left\{\max_{\mathbf{S}\subset \passage, |\mathbf{S}|=|\realAnswer|} {Sim}(\mathbf{S}, \realAnswer)>\alpha, \passage \in \filteredContextSet[\question]^+\right\}\,\,\,\nonumber
        \\
        \filteredContextSet[\question]^{--} = 
        \left\{\max_{\mathbf{S}\subset \passage, |\mathbf{S}|=|\realAnswer|} {Sim}(\mathbf{S}, \realAnswer)<\beta, \passage \in \filteredContextSet[\question]^-\right\}.\nonumber
        % \\
        % \label{eq:negative_samples}
        % \filteredContextSet[\question]^{--} = 
        % \filteredContextSet[\question]^-
        % \cap
        % \{\passage|Rouge\text{-}L(\passage, \realAnswer)<\beta\}
        % \filteredContextSet[\question]^{--} = 
        % \{\passage|Rouge\text{-}L(\passage, \realAnswer)<\beta, \passage \in \filteredContextSet[\question]^- \}
    \end{align}
}%
$\mathbf{S}$ is a span in $\passage$, $Sim(\cdot,\cdot)$ is Rouge-L between two sequences. $\alpha$ and $\beta$ are hyperparameters.




\paragraph{Method 2: Unsupervised ICT Training}
Inspired by the effectiveness of Inverse Cloze Task (ICT) \cite{Lee_2019orqa} as an unsupervised ranker training objective, we use it to pre-train our ranker. The rationale is that we construct ``pseudo-question'' $q$ and ``pseudo-evidence'' $b$ from the same original passage $p$ and aim at maximizing the probability $P_{\mathrm{ICT}}(b | q)$ of retrieving $b$ given $q$, which is estimated using negative sampling as:
\begin{equation}
    \small
    P_{\mathrm{ICT}}(b | q)
    =
    \frac{\exp \left(S_{r e t r}(b, q)\right)}{\sum_{b^{\prime} \in B} \exp \left(S_{r e t r}\left(b^{\prime}, q\right)\right)}.
\end{equation}
$S_{retr}(\cdot,q)$ is the relevance score between a paragraph and the ``pseudo-question'' $q$. $b'$$\neq$$b$ is sampled from original passages other than $p$. 

The selection of ``pseudo-questions'' is critical to ICT training. To select representative questions, we investigate several filtering methods, and finally develop a book-specific filter \footnote{A unique filter is built for each book.}. Our method selects the top-scored sentence in a passage as a ``pseudo-question'' in terms of its total of token-wise mutual information against the corresponding book. The details can be found in Appendix~\ref{app:detail_ORQA}.

% To welcome the questions that are closely correlated with its surrounding context, we develop a book-specific filter that only selects the top-scored sentence in a passage as a ``pseudo-question'' in terms of its total of word-wise mutual information against the corresponding book. 
% Besides, a minimum length constraint is applied; stopwords and punctuation are removed; \textcolor{red}{$90\%$ of the examples remove the sentence from the context following \cite{Lee_2019orqa}.}


%%%%%%  VERSION 2  %%%%%% 
% Recently in ODQA, the unsupervised per-training method, Inverse Cloze Task (ICT), has proven effective in helping the ranker model~\cite{Lee_2019orqa, guu2020realm}.
% % it is notoriously hard to train the ranker model in an end-to-end way, considering the large search space. 
% % One widely used technique these days is to first pre-train the QA model using weak supervision and then fine-tune it over the target QA datset.
% % Inspired by this, we use the Inverse Cloze Task (ICT) proposed in \cite{Lee_2019orqa}
% % \footnote{There is an improved 
% % Bayesian version of ICT pre-training task proposed by \cite{guu2020realm}. But due to the limitation on computational resources, we cannot conduct such pre-training.} 
% % to pre-train our BERT ranker.
% Inspired by this, we also study the usage of ICT to pre-train our ranker. ICT requires the model to predict which passage the given sentence comes from. 
% % It is an unsupervised analogy of supervised evidence retrieval task in that, 
% The rationale behind this is that we can view the extracted sentence as ``pseudo-question'' and view the source passage as ``pseudo-evidence''.
% % 
% Specifically, ICT aims at maximizing the probability $P_{\mathrm{ICT}}(b | q)$ of retrieving ``pseudo-evidence'' $b$ based on ``pseudo-question'' $q$, which is estimated using negative sampling as:
% \begin{equation}
%     P_{\mathrm{ICT}}(b | q)
%     =
%     \frac{\exp \left(S_{r e t r}(b, q)\right)}{\sum_{b^{\prime} \in B} \exp \left(S_{r e t r}\left(b^{\prime}, q\right)\right)}.
% \end{equation}
% where $S_{retr}(b,q)$ is the relevance score between ``pseudo-evidence'' $b$ and the ``pseudo-question'' $q$. All $b' \neq b$ is the negative samples in each batch $B$. % $\mathrm{BATCH}$. 

% When generating pseudo QA samples, careful selection of ``pseudo-questions'' is critical. We observe that the ``pseudo-questions'' whose answers are closely correlated with the preceding and training context, are useful. To exclude the ``nonsense pseudo-questions'', we develop a book-specific filter that only selects the top-scored sentence in a passage as a ``pseudo-question'' based on its total word-level mutual information. The details of scoring algorithm and relevant pre-processing can be found in Appendix \ref{app:detail_ORQA}.


%%%%%%  VERSION 1  %%%%%% 
% However, in our pilot experiments, we find that we can not naively apply ICT pretraining on BookQA. We have to take care about picking out ``pseudo-question'' because there are many random and casual statements or conversations in the books and does not bear strong relations with the context around. We use a word-level mutual-information based book-specific filtering techniques to filter out ``pseudo-question'', which score each ``pseudo-question'' is scored based on the sum of book-specific mutual information of words contained in the sentence. We only pick the top1 sentence in each passage as the ``pseudo-question'' and use the context as the ``pseudo-evidence''. Following the setting in \cite{Lee_2019orqa}, we only remove the sentence from its context in $90\%$ examples to keep the model learn basic lexical matching ability.



\paragraph{Method 3: Hard EM}
% We study the feasibility of Hard EM for ranker training. 
Hard EM is an iterative learning scheme. It was first introduced to ODQA by \citet{min2019discrete}, to find correct answer spans that maximize the reader performance.
% \footnote{As shown in~\cite{yang2020improving}, the Hard EM objective is related to policy gradient. Therefore, we categorize \cite{min2019discrete} and \cite{wang2018r} to the same class.} 
Here we adapt the algorithm to ranker training.
Specifically, the hard EM can be achieved in two steps. At step $t$, the E-step first trains the reader with the current top-$k$ selections ${\filteredContextSet[Q]}^t$ as input to update its parameters $\Phi^{t+1}$; then derives the new positive passages ${\filteredContextSet[Q]^{+}}^{t+1}$ that maximizes the reader $\Phi^{t+1}$'s probability of predicting $\realAnswer$ (Eq.~\ref{eq:hardem_e2}).
The M-step updates the ranker parameter $\Theta$ (Eq.~\ref{eq:hardem_m}):

% learning an improved ranker measure $\Phi$ (Eq.~\ref{eq:hardem_e1} \& \ref{eq:hardem_e2}). 
\par 
\vspace*{-5mm}
{\small
    \begin{align} 
        \label{eq:hardem_e2}
        {\filteredContextSet[Q]^{+}}^{t+1} &= k\text{-}\max_{\passage \in \contextSet} P(\realAnswer | \passage, \Phi^{t+1})   \\
        \label{eq:hardem_m}
        \Theta^{t+1} &= \argmax_{\Theta} P({\filteredContextSet[Q]^+}^{t+1} | \Theta^t).
    \end{align}
}%
% \par 
% \vspace*{-5mm}
% {\small
%     \begin{align} 
%         \label{eq:hardem_e1}
%         \filteredContextSet[Q]^* &=  \argmax_{\filteredContextSet[Q]} P(\filteredContextSet[Q] | \Theta^t)       \\
%         \label{eq:hardem_e2}
%         \Phi^{t} &= \argmax_{\Phi} P(\proposedAnswer | \filteredContextSet[Q]^*, \Phi^{t-1})  \\
%         \label{eq:hardem_m}
%         \Theta^{t+1} &= \argmax_{\Theta} P(\filteredContextSet[Q] | \Theta^t, \Phi^{t})
%     \end{align}
% }%
In practice, \citet{min2019discrete} find that initialized with standard maximum likelihood training, the Hard EM usually converges in 1-2 EM iterations.  
% requires tremendous amount of resources, and we are only able to run the complete cycle once due to limited time and computational power.

% Different from the usage of hard EM in \cite{min2019discrete}, we use the idea to iteratively \emph{update the ranker instead of the reader}. This purpose is similar to \cite{wang2018r}. The hard EM can be potentially used to update our reader as well but.

%%%%%%  VERSION 1  %%%%%% 
% An alternate approach for ranker training is \textbf{Hard EM} as used in~\cite{min2019discrete}. They propose an iterative learning scheme for finding correct answer span from multiple candidates. The method can be adapted to the ranker-reader framework.\footnote{As shown in~\cite{yang2020improving}, the derived Hard EM training objective is related to policy gradient~\cite{williams1992simple}. Therefore, we categorize this and \cite{wang2018r} as the same class of methods.} Specifically, the Hard-EM first trains an initial ranker and reader. Then it derives the supervised labels for the ranker based on the reader's performance. We defer the algorithm details to Appendix \ref{app:hard_em}. In practice, this training scheme requires tremendous amount of resources, and we are only able to run the complete cycle once due to limited time and computational power.

% \begin{figure*}[ht!]%[width=\textwidth]
%     \small
%     \fontsize{8}{10.5}\selectfont
%     \centering
%     \begin{tabular}{
%             C{0.35\textwidth}
%             C{0.15\textwidth}
%             C{0.15\textwidth}
%             C{0.25\textwidth}}
%         \toprule
%         \textbf{System} & \textbf{w/ trained ranker} & \textbf{w/ pre-trained LM} & \textbf{w/ extra training data} \\
%         \midrule
%         \textcolor{red}{Attention Sum}/\textcolor{blue}{BiDAF} \cite{kovcisky2018narrativeqa}& & &\\
%         % \textcolor{blue}{BiDAF} \cite{kovcisky2018narrativeqa} & &\\
%         \textcolor{red}{IAL-CPG} \cite{tay2019simple}&  & &    \\
%         \textcolor{blue}{R$^3$} \cite{wang2018r}& $\checkmark$ & & \\
%         \textcolor{blue}{BERT-heur} \cite{frermann-2019-extractive} &  $\checkmark$ & $\checkmark$ & $\checkmark$\\
%         Our \textcolor{red}{generative}/\textcolor{blue}{extractive} systems & $\checkmark$ & $\checkmark$ & \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-2mm}
%     \caption{\small{Summary of the characteristics of the compared systems. \textcolor{red}{Red}/\textcolor{blue}{blue} color refers to generative/extractive QA systems. In addition to the standard techniques, \cite{wang2018r} uses reinforcement learning to train the ranker; and \cite{tay2019simple} uses curriculum to train the reader to overcome the divergence of evidence retrieval qualities between training and testing.}}
%     \vspace*{-2mm}
%     \label{fig:model_cheatsheet}
% \end{figure*}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
% %%%%%%%%%%%%%%%%  Experiments  %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Experimental Settings}

% \subsection{Dataset}
% All our experiments are conducted on NarrativeQA dataset \cite{kovcisky2018narrativeqa}. It has a collection of 783 books and 789 movie scripts and the same number of summaries, with each book or movie script containing an average of 62k words and each summary containing over 1,100 tokens on average. Besides, each document has 30 question-answer pairs generated by human annotators in free-form natural language. Hence, the answers are not guaranteed to appear in the books. NarrativeQA provides two different settings, the \textbf{summary} setting and the \textbf{full-story} setting. Our Book QA task corresponds to the full-story setting with the assumption that a summary doesn't exist.

% All raw data are preprocessed with SpaCy\footnote{\url{https://spacy.io/}} tokenization. Considering the variable length of the paragraphs in story and movie scripts, we reorganize the original paragraphs and split them into a sequence of non-overlapping trunks of a length of 200 tokens following~\cite{kovcisky2018narrativeqa}.


% \subsection{Baseline}\label{ssec:baseline}
% For evidence retrieval, we compare our weakly supervised BERT ranker to a baseline BM25 ranker. Apart from that, a strong ranker~\cite{frermann-2019-extractive} with additional supervision is compared in our experiments as a weak upper bound. The model is trained with unexpected help from the summary of the book which is considered unavailable by design in the Book QA setting and also the general full-story scenario where questions should be answered only from books. We take it as a weak upper bound, because the summary is written by human and can be viewed as human comprehension input. For the reader, we take a set of competitive generative and extractive baselines from \cite{kovcisky2018narrativeqa, frermann-2019-extractive, tay2019simple} under Narrative full-story setting.\footnote{The full-story setting corresponds to the Book QA task.} To show the properties of our readers, we also report our QA performance on the summary as supplementary information.

% \subsection{Metrics}
% Following previous works~\cite{kovcisky2018narrativeqa,tay2019simple,frermann-2019-extractive,min2019discrete}, we use Rouge-L~\cite{lin-2004-rouge} as the main metric for both evidence retrieval and question answering.\footnote{For fair comparison, we lowercase the answers and remove the punctuation, and utilize an open-source evaluation library~\cite{sharma2017nlgeval} from \url{https://github.com/Maluuba/nlg-eval}.} For completeness, in Appendix \ref{sec:append_full_results} we also report results with the other metrics used in the previous works, including Bleu-1, Bleu-4~\cite{papineni2002bleu}, Meteor~\cite{banerjee2005meteor}, Rouge-L~\cite{lin-2004-rouge}, and the Exact Match (EM) and F1 scores that are commonly used for assessing ODQA models. Our approach achieves the best performance across all of the metrics.


% \subsection{Implementation}

% We use two V100 GPUs and 48 Xeon-E5 CPUs to run our experiments. For ranker, we use \texttt{bert-base-uncased} model\footnote{https://github.com/huggingface/transformers}. We find our best performance at $\alpha = 0.7$, $\beta = 0.3$ and $\sigma = 8$ (Section~\ref{ssec:model_ranker}). For readers, we use \texttt{gpt2-medium} and \texttt{bart-large} respectively and train with batch size 1 and use top-$k=3$ retrieved passages as inputs.


% \paragraph{Model Selection} 
% For the ranker, we use the average score of upper bound EM and Rouge-L of top-5 ranked paragraphs to select our best models; whereas for the reader, we refer to the overall quality of the generated or extracted answers on dev set with regards to Rouge-L and EM scores.






